HiTZ@Antidote: Argumentation-driven Explainable Artificial Intelligence for Digital Medicine

Providing high quality explanations for AI predictions based on machine learning is a challenging and complex task. To work well it requires, among other factors: selecting a proper level of generality/specificity of the explanation; considering assumptions about the familiarity of the explanation beneficiary with the AI task under consideration; referring to specific elements that have contributed to the decision; making use of additional knowledge (e.g. expert evidence) which might not be part of the prediction process; and providing evidence supporting negative hypothesis. Finally, the system needs to formulate the explanation in a clearly interpretable, and possibly convincing, way. Given these considerations, ANTIDOTE fosters an integrated vision of explainable AI, where low-level characteristics of the deep learning process are combined with higher level schemes proper of the human argumentation capacity. ANTIDOTE will exploit cross-disciplinary competences in deep learning and argumentation to support a broader and innovative view of explainable AI, where the need for high-quality explanations for clinical cases deliberation is critical. As a first result of the project, we publish the Antidote CasiMedicos dataset to facilitate research on explainable AI in general, and argumentation in the medical domain in particular.

==> Makefile <==
# LATEX: pdflatex | xelatex | lualatex
LATEX = lualatex
LATEX_FLAGS = -shell-escape
BIBTEX = bibtex

FILES = $(patsubst %.tex, %.pdf, $(wildcard *.tex))

all: $(FILES)


%.pdf: %.tex
	$(LATEX) $(LATEX_FLAGS) $<
	$(LATEX) $(LATEX_FLAGS) $<
	-$(BIBTEX) `basename $< .tex`
	$(LATEX) $(LATEX_FLAGS) $<
	$(LATEX) $(LATEX_FLAGS) $<
	$(LATEX) $(LATEX_FLAGS) $<
	qpdf --linearize --newline-before-endstream $@ /tmp/$@
	mv /tmp/$@ $@

clean:
	-rm -f *.{log,toc,tac,aux,dvi,ps,bbl,blg,tmp,nav,out,snm,vrb,rel,cut,abs,xmpi,xmpdata,*~}
	-rm -rf out _minted* auto
	for i in $(ALLSUBDIRS); do \
	    (cd $$i; make clean) || exit 1; \
	done
	-rm $(FILES)

cleanall: clean
	-rm -rf out auto

==> tags <==
!_TAG_FILE_FORMAT	2	/extended format; --format=1 will not append ;" to lines/
!_TAG_FILE_SORTED	1	/0=unsorted, 1=sorted, 2=foldcase/
!_TAG_OUTPUT_FILESEP	slash	/slash or backslash/
!_TAG_OUTPUT_MODE	u-ctags	/u-ctags or e-ctags/
!_TAG_PATTERN_LENGTH_LIMIT	96	/0 for no limit/
!_TAG_PROGRAM_AUTHOR	Universal Ctags Team	//
!_TAG_PROGRAM_NAME	Universal Ctags	/Derived from Exuberant Ctags/
!_TAG_PROGRAM_URL	https://ctags.io/	/official site/
!_TAG_PROGRAM_VERSION	0.0.0	//
%.pdf	Makefile	/^%.pdf: %.tex$/;"	t
ANTIDOTE Datasets	main.tex	/^\\subsection{ANTIDOTE Datasets}$/;"	u	section:Ongoing Work
Argumentation mining and generation	main.tex	/^\\subsection{Argumentation mining and generation}$/;"	u	section:Related Work
BIBTEX	Makefile	/^BIBTEX = bibtex$/;"	m
CasiMedicos	main.tex	/^\\paragraph{CasiMedicos} is a community and collaborative medical project run by$/;"	P	subsection:Ongoing Work""ANTIDOTE Datasets
Concluding Remarks	main.tex	/^\\section{Concluding Remarks}$/;"	s
Crosslingual Knowledge Transfer	main.tex	/^\\subsection{Crosslingual Knowledge Transfer}$/;"	u	section:Ongoing Work
Devlin19	references.bib	/^@inproceedings{Devlin19,$/;"	j
Evaluation	main.tex	/^\\subsection{Evaluation}$/;"	u	section:Methology and Work Plan
Explainable AI	main.tex	/^\\subsection{Explainable AI}$/;"	u	section:Related Work
FILES	Makefile	/^FILES = $(patsubst %.tex, %.pdf, $(wildcard *.tex))$/;"	m
Introduction	main.tex	/^\\section{Introduction}$/;"	s
LATEX	Makefile	/^LATEX = lualatex$/;"	m
LATEX_FLAGS	Makefile	/^LATEX_FLAGS = -shell-escape$/;"	m
Methology and Work Plan	main.tex	/^\\section{Methology and Work Plan}$/;"	s
Ongoing Work	main.tex	/^\\section{Ongoing Work}$/;"	s
Question Answering in the Medical Domain	main.tex	/^\\subsection{Question Answering in the Medical Domain}$/;"	u	section:Ongoing Work
Related Work	main.tex	/^\\section{Related Work}\\label{sec:related-work}$/;"	s
The SAEI Corpus	main.tex	/^\\paragraph{The SAEI Corpus} is a collection of differential diagnosis in$/;"	P	subsection:Ongoing Work""ANTIDOTE Datasets
Welbl2017CrowdsourcingMC	references.bib	/^@inproceedings{Welbl2017CrowdsourcingMC,$/;"	j
Work Plan	main.tex	/^\\subsection{Work Plan}$/;"	u	section:Methology and Work Plan
adadi2018peeking	references.bib	/^@article{adadi2018peeking,$/;"	a
all	Makefile	/^all: $(FILES)$/;"	t
alshomary2020target	references.bib	/^@inproceedings{alshomary2020target,$/;"	j
alshomary2021argument	references.bib	/^@article{alshomary2021argument,$/;"	a
arrieta2020explainable	references.bib	/^@article{arrieta2020explainable,$/;"	a
bar2020arguments	references.bib	/^@article{bar2020arguments,$/;"	a
biran2017explanation	references.bib	/^@inproceedings{biran2017explanation,$/;"	j
chen2019seeing	references.bib	/^@article{chen2019seeing,$/;"	a
clean	Makefile	/^clean:$/;"	t
cleanall	Makefile	/^cleanall: clean$/;"	t
clinciu2021study	references.bib	/^@article{clinciu2021study,$/;"	a
doshi2017towards	references.bib	/^@article{doshi2017towards,$/;"	a
dusmanu2017argument	references.bib	/^@inproceedings{dusmanu2017argument,$/;"	j
eger2017neural	references.bib	/^@article{eger2017neural,$/;"	a
fig:scenario	main.tex	/^  \\label{fig:scenario}$/;"	l
fig:xai-darpa	main.tex	/^  \\label{fig:xai-darpa}$/;"	l
garcia-ferrero-etal-2022-model	references.bib	/^@inproceedings{garcia-ferrero-etal-2022-model,$/;"	j
gilpin2018explaining	references.bib	/^@inproceedings{gilpin2018explaining,$/;"	j
gunning2019xai	references.bib	/^@article{gunning2019xai,$/;"	a
hidey2019fixed	references.bib	/^@inproceedings{hidey2019fixed,$/;"	j
hua2018neural	references.bib	/^@article{hua2018neural,$/;"	a
hua2019argument	references.bib	/^@article{hua2019argument,$/;"	a
jin2021disease	references.bib	/^@article{jin2021disease,$/;"	a
johnson2012manifest	references.bib	/^@book{johnson2012manifest,$/;"	b
kayser2021vil	references.bib	/^@inproceedings{kayser2021vil,$/;"	j
kim2018textual	references.bib	/^@inproceedings{kim2018textual,$/;"	j
klebanov2016argumentation	references.bib	/^@inproceedings{klebanov2016argumentation,$/;"	j
levy2014context	references.bib	/^@inproceedings{levy2014context,$/;"	j
lipton2018mythos	references.bib	/^@article{lipton2018mythos,$/;"	a
liu2021synthetic	references.bib	/^@article{liu2021synthetic,$/;"	a
mayer2019acta	references.bib	/^@inproceedings{mayer2019acta,$/;"	j
mayer2021enhancing	references.bib	/^@article{mayer2021enhancing,$/;"	a
miller2019explanation	references.bib	/^@article{miller2019explanation,$/;"	a
nguyen2018argument	references.bib	/^@inproceedings{nguyen2018argument,$/;"	j
park2019generating	references.bib	/^@inproceedings{park2019generating,$/;"	j
persing2016end	references.bib	/^@inproceedings{persing2016end,$/;"	j
rinott2015show	references.bib	/^@inproceedings{rinott2015show,$/;"	j
sato2015end	references.bib	/^@inproceedings{sato2015end,$/;"	j
schiller2020aspect	references.bib	/^@article{schiller2020aspect,$/;"	a
sec:related-work	main.tex	/^\\section{Related Work}\\label{sec:related-work}$/;"	l
singhal2022large	references.bib	/^@inproceedings{singhal2022large,$/;"	j
slonim2021autonomous	references.bib	/^@article{slonim2021autonomous,$/;"	a
soldaini2016quickumls	references.bib	/^@inproceedings{soldaini2016quickumls,$/;"	j
stab2017parsing	references.bib	/^@article{stab2017parsing,$/;"	a
stab2018cross	references.bib	/^@article{stab2018cross,$/;"	a
wang2016neural	references.bib	/^@article{wang2016neural,$/;"	a
xue-etal-2021-mt5	references.bib	/^@inproceedings{xue-etal-2021-mt5,$/;"	j
yang2018hotpotqa	references.bib	/^@article{yang2018hotpotqa,$/;"	a
yeginbergenova2023crosslingual	references.bib	/^@inproceedings{yeginbergenova2023crosslingual,$/;"	j
zhangbertscore	references.bib	/^@inproceedings{zhangbertscore,$/;"	j

